MMT: A Multilingual and Multi-Topic Indian Social Media Dataset

Social media plays a significant role in cross-cultural communication. A vast amount of this occurs in code-mixed and multilingual form, posing a significant challenge to Natural Language Processing (NLP) tools for processing such information, like language identification, topic modeling, and named-entity recognition. To address this, we introduce a large-scale multilingual, and multi-topic dataset (MMT) collected from Twitter (1.7 million Tweets), encompassing 13 coarse-grained and 63 fine-grained topics in the Indian context. We further annotate a subset of 5,346 tweets from the MMT dataset with various Indian languages and their code-mixed counterparts. Also, we demonstrate that the currently existing tools fail to capture the linguistic diversity in MMT on two downstream tasks, i.e., topic modeling and language identification. To facilitate future research, we have make the anonymized and annotated dataset available at https://huggingface.co/datasets/LingoIITGN/MMT.

==> tables/lang_data.tex <==
\begin{table}[!tbh]
\centering
\small{
\begin{tabular}{lcccc}
\toprule
\textbf{Language}& \textbf{Tweets} & \textbf{Correct} & \textbf{En} &  \textbf{Hi} \\ \hline

\textit{En} &   3907  &    3716  &  3696    &  38   \\ 
\textit{En-Hi}&   459  &     0     &    119    &     200\\ 
\textit{Hi}      &     418& 325 &   29     &   311  \\ 
\textit{Gu}&   51  &      45    &  2      & 2   \\ 
\textit{Bn}
 &    44 &    42      & 0& 2    \\ 
All CMs & 612&   0   &    142
    &  205  \\ 

\bottomrule
\end{tabular}}
\caption{Distribution of language annotation by human annotators in the \textit{MMT-LID} dataset. Here, we report the top-5 identified languages by the human annotators in the \textit{MMT-LID} dataset. Here, Correct shows the number of tweets with correct language identification by Twitter. En and Hi shows the language identified by twitter.}
\label{tab: lang_data}
\end{table}

==> tables/likes_count.tex <==
\begin{table}[]
\begin{tabular}{|r|r|lll}
\cline{1-2}
\textbf{topic\_name}                & \textbf{likes\_count}       &  &  &  \\ \cline{1-2}
Education                           & 9.365                       &  &  &  \\ \cline{1-2}
Journalism \& Media                 & 12.575                      &  &  &  \\ \cline{1-2}
Manufacturing                       & 10.306                      &  &  &  \\ \cline{1-2}
Sports                              & 23.883                      &  &  &  \\ \cline{1-2}
R\&D and Technology                 & 11.918                      &  &  &  \\ \cline{1-2}
Politics                            & 19.454                      &  &  &  \\ \cline{1-2}
Art and Literature                  & 14.790                      &  &  &  \\ \cline{1-2}
Natural Disaster                    & 13.354                      &  &  &  \\ \cline{1-2}
Economics and Retail                & 10.277                      &  &  &  \\ \cline{1-2}
FOOD                                & 6.029                       &  &  &  \\ \cline{1-2}
ENVIRONMENT                         & 12.698                      &  &  &  \\ \cline{1-2}
Wildlife and Vegetation             & 9.815                       &  &  &  \\ \cline{1-2}
\multicolumn{1}{|l|}{Films and OTT} & \multicolumn{1}{l|}{33.440} &  &  &  \\ \cline{1-2}
\end{tabular}
\end{table}

==> tables/replies_count.tex <==

\begin{table}[]
\begin{tabular}{|r|r|lll}
\cline{1-2}
\textbf{topic\_name}                & \textbf{replies\_count}    &  &  &  \\ \cline{1-2}
Education                           & 0.610                      &  &  &  \\ \cline{1-2}
Journalism \& Media                 & 0.718                      &  &  &  \\ \cline{1-2}
Manufacturing                       & 0.425                      &  &  &  \\ \cline{1-2}
Sports                              & 0.875                      &  &  &  \\ \cline{1-2}
R\&D and Technology                 & 0.657                      &  &  &  \\ \cline{1-2}
Politics                            & 0.947                      &  &  &  \\ \cline{1-2}
Art and Literature                  & 0.780                      &  &  &  \\ \cline{1-2}
Natural Disaster                    & 0.707                      &  &  &  \\ \cline{1-2}
Economics and Retail                & 0.709                      &  &  &  \\ \cline{1-2}
FOOD                                & 0.803                      &  &  &  \\ \cline{1-2}
ENVIRONMENT                         & 0.685                      &  &  &  \\ \cline{1-2}
Wildlife and Vegetation             & 0.437                      &  &  &  \\ \cline{1-2}
Films and OTT & 2.340 &  &  &  \\ \cline{1-2}
\end{tabular}
\end{table}

==> tables/retweet_count.tex <==
\begin{table}[]
\begin{tabular}{|r|r|lll}
\cline{1-2}
\textbf{topic\_name}    & \textbf{retweets\_count} &  &  &  \\ \cline{1-2}
Education               & 6.119                    &  &  &  \\ \cline{1-2}
Journalism \& Media     & 3.095                    &  &  &  \\ \cline{1-2}
Manufacturing           & 2.871                    &  &  &  \\ \cline{1-2}
Sports                  & 2.322                    &  &  &  \\ \cline{1-2}
R\&D and Technology     & 2.773                    &  &  &  \\ \cline{1-2}
Politics                & 9.196                    &  &  &  \\ \cline{1-2}
Art and Literature      & 3.155                    &  &  &  \\ \cline{1-2}
Natural Disaster        & 3.033                    &  &  &  \\ \cline{1-2}
Economics and Retail    & 2.375                    &  &  &  \\ \cline{1-2}
FOOD                    & 1.113                    &  &  &  \\ \cline{1-2}
ENVIRONMENT             & 4.386                    &  &  &  \\ \cline{1-2}
Wildlife and Vegetation & 2.599                    &  &  &  \\ \cline{1-2}
Films and OTT           & 3.993                    &  &  &  \\ \cline{1-2}
\end{tabular}
\end{table}
